Chirality inversion and odd transport in a suspension of living rotors

Chiral symmetry breaking is a defining feature of life, visible at all scales from molecules to organisms. Yet how microscopic chirality propagates to shape the macroscopic properties of living matter remains poorly understood. Here, using a new experimental system of spinning microalgae, we show that a living chiral fluid behaves fundamentally differently from an externally driven one. As their density increases, cells self-assemble hydrodynamically into small rotating clusters which merge into a percolating chiral fluid. Strikingly, microscopic and macroscopic vorticity have opposite signs: individual cells all spin clockwise, yet clusters orbit counterclockwise. Combining experiments, theory and simulations, we show that both chirality inversion and percolation are direct consequences of the cells' internally driven nature. We then show how percolation reshapes transport, with even and odd diffusivities responding differently to the emerging network topology.

==> colors_define.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\definecolor{darkorange}{rgb}{1.0, 0.55, 0.0}
\definecolor{persiangreen}{rgb}{0.0, 0.65, 0.58}
\definecolor{persianindigo}{rgb}{0.2, 0.07, 0.48}
\definecolor{cadet}{rgb}{0.33, 0.41, 0.47}
\definecolor{turquoisegreen}{rgb}{0.63, 0.84, 0.71}
\definecolor{sandybrown}{rgb}{0.96, 0.64, 0.38}
\definecolor{blueblue}{rgb}{0.0, 0.2, 0.6}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{greengreen}{rgb}{0.0, 0.5, 0.0}


\definecolor{saffron}{rgb}{0.96, 0.77, 0.19}
\definecolor{urobilin}{rgb}{0.88, 0.68, 0.13}
\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\definecolor{brass}{rgb}{0.71, 0.65, 0.26}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{denim}{rgb}{0.08, 0.38, 0.74}
\definecolor{niceRed3}{RGB}{199,19,19}

==> fig_methodimages.tex <==

%\tdplotsetmaincoords{60}{130}
%\tdplotsetmaincoords{60}{120}
%\tdplotsetmaincoords{70}{110}
\tdplotsetmaincoords{70}{105}

%\tdplotsetmaincoords{60}{130}

\begin{tikzpicture}[tdplot_main_coords,>=latex,scale=1.5]

  \draw[->] (0,0,0) -- (3,0,0) node[anchor=north east]{$x$};
  \draw[->] (0,0,0) -- (0,3,0) node[anchor=west]{$y$};
  \draw[->] (0,0,0) -- (0,0,2) node[anchor=south]{$z$};

\fill[gray,very nearly transparent] (0,0,1) -- (0,3,1) --(3,3,1)  --(3,0,1)-- cycle ;
%\fill[gray,very nearly transparent] (0,0,-1) -- (0,3,-1) --(3,3,-1)  --(3,0,-1)-- cycle ;





\coordinate (Tr) at (1.5,1,1);
\coordinate (F1r) at (1.5,1,1);
\coordinate (F2r) at (1.5,2,1);
\coordinate (Ti) at (1.5,1,-1);
\coordinate (F1i) at (1.5,1,-1);
\coordinate (F2i) at (1.5,2,-1);

\coordinate (Obs) at (.5,2.5,1);
\draw[ ->] (F2r) -- (Obs)node[anchor=north,scale=1,pos=.5,above] {$\vec{r}'$};
\draw[thin, ->] (F2i) -- (Obs)node[anchor=north,scale=1,pos=.5,rotate=70] {$\vec{r}'_*$};

\draw[very thin, dashed,black] (Tr)-- ++(0,0,-1); %--($(Ti)-(0,0,1)$);
\draw[very thin, dashed,black] (F2r)-- ++(0,0,-1);
\draw[very thin, dotted,black] (Ti)-- ++(0,0,1); %--($(Ti)-(0,0,1)$);
\draw[very thin, dotted,black] (F2i)-- ++(0,0,1);


%Real system
\begin{scope}[canvas is xy plane at z=1]

   \coordinate (O) at (1.5,1);
    \coordinate (L) at (1.5,2);
    \coordinate (F) at (L) ++(-80:.7);


      \draw[bleudefrance,very thick,
       decoration={markings, mark=at position .2 with {\arrow[yshift=0.33\pgflinewidth, bleudefrance]{>}}},postaction={decorate}
      ] (O) circle(.3); 

\draw[very thick,Red3 , ->] (O) -- ++(170:.8)node[anchor=south,scale=.7] {$\bm F_1$};
\draw[very thick,Red3 , ->] (L) -- ++(-10:.8)node[anchor=north,scale=.7] (F2) {$\bm F_2$};
\draw[very thick] (O) -- (L)node[anchor=north,scale=1,pos=.5] {$l$};
\end{scope}

%Image system
\begin{scope}[canvas is xy plane at z=-1]

   \coordinate (Oi) at (1.5,1);
    \coordinate (Li) at (1.5,2);
    \coordinate (Fi) at (L) ++(-80:.7);

    \draw[bleudefrance!50,very thick,
    decoration={markings, mark=at position .2 with {\arrow[yshift=0.33\pgflinewidth,bleudefrance!50]{<}}},postaction={decorate}
    ] (Oi) circle(.3); 
    \draw[very thick,Red3!50 , ->] (Oi) -- ++(170+180:.8)node[anchor=south,scale=.7] {$\bm F_1$};
    \draw[very thick,Red3!50 , ->] (Li) -- ++(-10+180:.8)node[anchor=north,scale=.7] (F2il) {$\bm F_2$};
\end{scope}


\shade[ball color=Red3!50] ($(Ti)-(0,0,1)+(-10:.07)$) circle (.2ex);
\shade[ball color=Red3!50] ($(Ti)-(0,0,1)+(-10+180:.07) $) circle (.2ex);

\shade[ball color=Red3!50] ($(F2i)-(0,0,1)+(-10:.07)$) circle (.2ex);
\shade[ball color=Red3!50] ($(F2i)-(0,0,1)+(-10+180:.07) $) circle (.2ex);
\draw[Red3!50,thick,->] ($(F2i)-(0,0,.5)+(0,0,-.15)+(-10+180:.07) $) -- ++(0,0,0.3);
\draw[Red3!50,thick,->] ($(F2i)-(0,0,.5)+(0,0,.15)+(-10:.07) $) -- ++(0,0,-0.3);

\draw[Red3!50,thick,->] ($(Oi)-(0,0,.5)+(0,0,-.15)+(-10+180:.07) $) -- ++(0,0,0.3);
\draw[Red3!50,thick,->] ($(Oi)-(0,0,.5)+(0,0,.15)+(-10:.07) $) -- ++(0,0,-0.3);
  
 
\shade[ball color=black] (Tr) circle (.2ex);
\shade[ball color=black] (F2r) circle (.2ex);
\shade[ball color=gray] (Ti) circle (.2ex);
\shade[ball color=gray] (F2i) circle (.2ex);

\fill[gray,nearly transparent] (0,0,0) -- (0,3,0) --(3,3,0)  --(3,0,0)-- cycle ;
  
\end{tikzpicture}



==> fig_rotationalavg.tex <==

\begin{tikzpicture}[scale=2,>=Latex]

\begin{scope}    
    \node[opacity=.56,scale=.08,rotate=28] (image) at (0,0){\includegraphics{chlamyBG2.png}};
\end{scope}


    \coordinate (O) at (0,0);
    \draw[thin,->,gray] (O) -- ++(1.5,0)node[anchor=north,scale=1] {$x$};
    \draw[thin,->,gray] (O) -- ++(0,1.5)node[anchor=west,scale=1] {$y$};

\begin{scope} [rotate=50]    
    \coordinate (L) at (1,0);
    \coordinate (L2) at (2,0);
    \coordinate (F) at (L) ++(-80:.7);
    \draw[very thick,bleudefrance , ->] (-.2,0) arc (180:360+180:.2)node[anchor=east,scale=1] {$\bm T$};
    \draw[very thick,Red3 , ->] (O) -- ++(80:.7)node[anchor=east,scale=1] {$\bm F_1$};
    \draw[very thick,Red3 , ->] (L) -- ++(-100:.7)node[anchor=north,scale=1] (F2) {$\bm F_2$};
    \draw[very thick] (O) -- (L)node[anchor=north,above,scale=1,pos=.5] {$l$};
    %\draw[thin,gray] (L) -- ++(.2,0);
    \filldraw [black] (O) circle (.5pt);
    \filldraw [black] (L) circle (.5pt);
    \path (O) -- (L) -- (F2)
pic (delta) [draw, thin,angle radius=.3cm] {angle = O--L--F2};
\node[scale=1,black] (etaL) at ($(L)+(-140:.3)$) {$\alpha$};
\end{scope} 

%%%%%%%%%%%%%%%%%%%%%%%%5



\begin{scope}
\clip(-.4,-.3) rectangle (3.5,2.5);
   

\node[inner sep=0,outer sep =0] (O) at (0,0){};
\node[inner sep=0,outer sep =0] (arm) at (2,2){};
\node[inner sep=0,outer sep =0] (obv) at (2.7,1){};
\node[inner sep=0,outer sep =0] (C) at (0,.5){};
\node[inner sep=0,outer sep =0] (M) at (L){} ;
\filldraw [black] (obv) circle (.5pt);
\draw[arrows = {-Latex[scale=.5]},scale=.7] (M) -- ([turn]90:.45cm) coordinate (T) node[anchor=south east,scale=1,black] {$\hat t$};
\draw[arrows = {-Latex[scale=.5]},scale=.7] (M) -- ([turn]0:.45cm)  coordinate (N) node[anchor=south west,scale=1,black] {$\hat n$};
\node[draw,very thin,dashed, gray] at (0,0) [circle through={(M)}] {}; 

\draw[very thin,gray] (0,0) -- (obv) node[anchor=west,scale=1,black,pos=.75,below,sloped] {$\vec{r}$};
\draw[very thin,gray] (M) -- (obv) node[anchor=west,scale=1,black,pos=.5,above,sloped] {$\vec{r}'$};

\path (1,0) coordinate (X) -- (O) -- (obv)
    pic (thet) [draw,very thin,angle radius=1cm] {angle = X--O--obv};
\path (1,0) coordinate (X) -- (O) -- (M)
    pic (thet) [draw,very thin,angle radius=.7cm] {angle = X--O--M};
\node[scale=.7,black] (omegat) at (.35,.25) {$\omega\, t$};
\node[scale=.6,black] (theta) at (.7,.1) {$\theta$};


\path (arm) -- (M) -- (N)
    pic (eta) [draw,very thin,angle radius=.45cm] {angle = arm--M--N};


\end{scope}

\end{tikzpicture} 


==> tikz_definitions.tex <==
\usepackage{tikz}

\usetikzlibrary{calc,patterns,arrows,shapes,arrows,intersections,decorations,shadows,shapes.geometric,angles,through,quotes}
\usetikzlibrary{patterns,arrows,shapes,shapes.arrows,arrows,intersections,decorations,shadows,backgrounds}
\usetikzlibrary{spy,angles,quotes}
\usetikzlibrary{patterns,arrows,shapes,arrows,intersections,decorations}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta, decorations.text}

\usetikzlibrary{decorations.markings}


\usepackage{tikz-3dplot}
\usepackage{circuitikz}

%\usepackage{caption}
%\usepackage{subcaption}


\usepackage{braket}
\usetikzlibrary{patterns,arrows,shapes,arrows,intersections,decorations}
\usetikzlibrary{angles,quotes} % for pic
\usepackage{pgfplots}
%\pgfplotsset{compat=1.9}
\usepgfplotslibrary{fillbetween}

\usepackage{pgfgantt}

